Using Motion Cues to Supervise Single-Frame Body Pose and Shape Estimation in Low Data Regimes

When enough annotated training data is available, supervised deep-learning algorithms excel at estimating human body pose and shape using a single camera. The effects of too little such data being available can be mitigated by using other information sources, such as databases of body shapes, to learn priors. Unfortunately, such sources are not always available either. We show that, in such cases, easy-to-obtain unannotated videos can be used instead to provide the required supervisory signals. Given a trained model using too little annotated data, we compute poses in consecutive frames along with the optical flow between them. We then enforce consistency between the image optical flow and the one that can be inferred from the change in pose from one frame to the next. This provides enough additional supervision to effectively refine the network weights and to perform on par with methods trained using far more annotated data.

==> figs/loss_norm.tex <==
\begin{figure}
\centering
\begin{minipage}[l]{0.4\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/loss_norm_off.pdf}
\end{minipage}
%
\begin{minipage}[r]{0.4\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figs/loss_norm_on.pdf}
\end{minipage}
%
\caption{
   \small
   We found that the differences in motion behavior may drastically differ across different datasets or even same video sequences.
   On the {\it left}, we show the values of $L_{\OF}$ (Eq.~\ref{eq:lossOF2}
   ) for $2k$ samples of each of the video datasets. 
   We propose to normalize $L_{\OF}$ for every sample over the mean of the \OF{} norms across all visible vertices. The result is on the {\it right}.
   Loss normalization significantly stabilizes the training.
   }
\label{fig:loss_norm}
\end{figure}


==> figs/low_data_tp.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.45\textwidth]{figs/low_data_tp.pdf}
\end{center}
\vspace{-4mm}
   \caption{
   \small{{\bf Our method vs TexturePose.} We plot P-MPJPE as a function of the percentage of the annotations we used before refinement for the baseline model and after semi-supervised refinement using either TexturePose, our approach with \OF{} only, or both \OF{} and TexturePose. 
   Our approach outperforms TexturePose, and, as expected, the less annotated data we use, the greater the improvement.
   For video dataset, Human3.6M was used. 
   All metrics are P-MPJPE on 3DPW-test set.
   }}
\label{fig:low_data_tp}
\end{figure}

==> figs/missed_alignment.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.35\textwidth]{figs/missed_alignment.pdf}
\end{center}
   \caption{
   \small{{\bf Randomization.} The first  two columns in every row show pairs of consecutive frames from different video datasets, 3DPW, H36M and PennAction, with overlaid body estimates. These estimates are very similar to each other but wrong. The third column feature the body estimate for the second frame after color randomization. Even if this does not give the correct motion flow or \OF{}, it disentangles body estimates from each other.}}
\label{fig:missed_alignment}
\end{figure}

==> figs/of_branch.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.47\textwidth]{figs/of_branch.pdf}
\end{center}
\vspace{-4mm}
   \caption{
   \small{
   {\bf Self-supervised training with optical flow guidance.} 
   The upper branch illustrates the inference of the partially trained network. 
   It yields SMPL body mesh estimates $\bm{B}_1$ and $\bm{B}_2$ for two consecutive frames $\bI_1$ and $\bI_2$ of an unlabeled video sequence. 
   Both are projected into the image space to obtain per-vertex pixel coordinates. 
   The per-vertex displacement between them is denoted as $\mathbf{F}_{\bm{B}}$.
   The lower branch involves optical flow evaluation. 
   The optical flow map \OF{} estimated from $\bI_1$ and $\bI_2$ is sampled at the coordinates $\bm{\Pi}(\bm{B}_1)$ to derive $\OF$ values for every vertex by 2D bilinear interpolation. 
   The resulting per-vertex map is denoted as $\mathbf{F}_{\OF}$.
   We then minimize the distance between $\mathbf{F}_{\OF}$ and $\mathbf{F}_{\bm{B}}$.
   }}
\label{fig:of_branch}
\end{figure}

==> figs/unannot_data.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.45\textwidth]{figs/unannot_data_.pdf}
\end{center}
\vspace{-4mm}
   \caption{\small 
   {{\bf More unlabelled videos.} 
   We plot P-MPJPE as a function of the amount of unlabelled data used for fine-tuning \BL{} using our approach. 
   As expected, the more unannotated data we use, the greater the improvement.
   All metrics are P-MPJPE on 3DPW-test set.
   }
   }
\label{fig:unannot_data}
\end{figure}


==> tabs/ft_w_coco.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[t]
\begin{small}
\begin{center}
\scalebox{1.05}{
\begin{tabular}{l|cc}
   & P-MPJPE ($\downarrow$) & Accel.Err ($\downarrow$) \\
  \hline
  H36M                & 57.1 & 24.4 \\
  H36M + 3DPW-tr      & 56.4 & 24.0 \\
  H36M + 3DPW-tr + PA & 56.2 & 23.9 \\
  \hline
  3DPW-test  & \textit{55.8} & \textit{20.2} \\
    \hline
\end{tabular}}
\end{center}
\end{small}
\vspace{-3mm}
\caption{\small {\bf More unannotated data.} 
Starting from the \BL{} pre-trained using \COCO{100}, 
we refine it using images from either H36M alone, or H36M and 3DPW-tr, or H36M, 3DPW-tr, and PA. 
As expected, the more images we use, the better the performance. 
The last row corresponds to using the test-set itself for supervision, 
which is meaningful and practical in some cases because the loss is self-supervised. 
This yields the best performance but using H36M + 3DPW-tr + PA comes close. 
}
\label{table:ft_w_coco}
\end{table}

==> tabs/low_data_tp.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}[t]
\begin{small}
\begin{center}
\scalebox{1.0}{
\begin{tabular}{l|c|ccc}
  \% of COCO$_{\text{EFT}}$ & \BL{} & TP & \OF{} & mix\\
  \hline
  \COCO{10}   & 65.3 & 62.7 & 61.3 & 60.4  \\
  \COCO{20}   & 62.2 & 60.0 & 59.3 & 58.7  \\
  \COCO{50}   & 59.4 & 58.8 & 58.0 & 57.6  \\
  \COCO{100} & 58.2 & 58.1 & 57.1 & 56.9  \\
    \hline
\end{tabular}}
\end{center}
\end{small}
\vspace{-4mm}
\caption{\small {\bf Fine-tuning the baseline model \BL{}} using our $\OF$-guided method, TexturePose~\citep{Pavlakos19b} (TP) and the mix of the two. 
For video dataset, Human3.6M was used. All metrics are P-MPJPE on 3DPW-test set.}
\label{table:low_data_tp}
\end{table}

==> tabs/single_frame_sota.tex <==
\begin{table}[t]
\begin{small}
\begin{center}
\scalebox{1.0}{
\begin{tabular}{l|cc}
    & P-MPJPE & Accel.Err \\
  \hline  
  \BL{} \big(\COCO{100}\big) & 58.2 & 29.0 \\
%
   SPIN{\scriptsize~\citep{Kolotouros19}}                & 59.2 & 29.8 \\
   PyMAF{\scriptsize~\citep{Zhang21b}}              & 58.9 & - \\
   I2L-MeshNet{\scriptsize~\citep{Moon20}}  & 57.7 & 30.9 \\
   \hline
   \OF{} \big(\COCO{100}\big) & 57.1 & 24.4 \\
   \OF{}+TP \big(\COCO{100}\big) & 56.9 & 24.1 \\
    \hline
    PARE{\scriptsize~\citep{Kocabas21}}} & 52.3 & - \\
    HybriK{\scriptsize~\citep{Li21i}} & 48.8 & - \\
    HMR2.0{\scriptsize~\citep{goel23}} & 44.4 & - \\
\end{tabular}
\end{center}
\end{small}
\caption{
{\bf Performance of state-of-the-art methods} for comparison purposes. 
All metrics are P-MPJPE on 3DPW-test set.
}
\label{table:single_frame_sota}
\end{table}

==> tex/limitations_and_future_work.tex <==
\section{Limitations and Future Work}


